MEKER: Memory Efficient Knowledge Embedding Representation for Link Prediction and Question Answering

Knowledge Graphs (KGs) are symbolically structured storages of facts. The KG embedding contains concise data used in NLP tasks requiring implicit information about the real world. Furthermore, the size of KGs that may be useful in actual NLP assignments is enormous, and creating embedding over it has memory cost issues. We represent KG as a 3rd-order binary tensor and move beyond the standard CP decomposition by using a data-specific generalized version of it. The generalization of the standard CP-ALS algorithm allows obtaining optimization gradients without a backpropagation mechanism. It reduces the memory needed in training while providing computational benefits. We propose a MEKER, a memory-efficient KG embedding model, which yields SOTA-comparable performance on link prediction tasks and KG-based Question Answering.

==> wiki5m.tex <==
\begin{table*}[tb]
\fontsize{9.0pt}{9.0pt}\selectfont%
\centering % used for centering table
\begin{tabular}{@{}lrrrrrr@{} } % centered columns (4 columns)
\toprule %inserts double horizontal lines
Model  & MRR & Hit@1 & Hit@3 & Hit@10 &  Memory, GB & Storage, GB  \\ % inserts table
\midrule % inserts single horizontal line

PTBG~(ComplEX)~\cite{pbg} & 0.184  & 0.131 & 0.210 & 0.287 & 45.15  & 9,25 \\

PTBG~(TransE)~\cite{pbg}  & 0.150  & 0.091 & 0.176 & 0.263 & 43.64  & 9,25\\

% TransR (Lin et al., 2015) & - & - & - & - & - & distance based model\\
MEKER~(ours) & \textbf{0.202} & \textbf{0.149} &\textbf{0.238}  & \textbf{0.325} & \textbf{24.27} & \textbf{0}\\
%MEKER first &0.143 & 0.129 & 0.199  & 0.279 & 24.3 \\
\bottomrule
\end{tabular}
\caption{Unfiltered link prediction scores for MEKER and PyTorchBigGraph approaches for Wiki4M dataset and memory needed in leveraging every model. Storage means additional memory demanded for auxiliary structures.}
\label{table:wiki5m} % is used to refer this table in the text
\end{table*}
